Unsupervised semantic discovery through visual patterns detection

We propose a new fast fully unsupervised method to discover semantic patterns. Our algorithm is able to hierarchically find visual categories and produce a segmentation mask where previous methods fail. Through the modeling of what is a visual pattern in an image, we introduce the notion of "semantic levels" and devise a conceptual framework along with measures and a dedicated benchmark dataset for future comparisons. Our algorithm is composed by two phases. A filtering phase, which selects semantical hotsposts by means of an accumulator space, then a clustering phase which propagates the semantic properties of the hotspots on a superpixels basis. We provide both qualitative and quantitative experimental validation, achieving optimal results in terms of robustness to noise and semantic consistency. We also made code and dataset publicly available.

==> sections/abstract.tex <==
\begin{abstract}
    Unsupervised image segmentation is a well-defined problem only when dealing with syntactic features. This is the case, for instance, when seeking for objects of similar colors or areas separated by sharp edges. When semantic comes into play, things become more and more slippery, as the binding between low-level appearance and segments is lost. Supervised methods would solve the issue by building a statistical model of the relevant objects to be segmented, being them people, trees or cars. Unsupervised approaches, by contrast, would need to automatically learn the models, however it is not clear which should be the implicit definition of an ``object'', neither how to set the correct hierarchical segmentation level, which can range from a tree as a whole to a single leaf.
    With this paper we try to solve this quandary in the special (but not uncommon) scenario where several complete or partial repetitions of similar subjects are found in the scene. The leading idea is that if a pattern is replicated consistently enough it has good chances of being a well defined object from a semantic standpoint.  
    Specifically, we introduce a fast algorithm to find, without any supervision, hierarchical visual categories from repeated similar pattern in images. In order to assess the quality of a segmentation spanning different levels of detail we introduce the notion of ``semantical levels'' and we devise a conceptual framework along with metrics and a dedicated benchmark dataset. The effectiveness of our method is then measured by performing both qualitative and quantitative experimental validations.

\end{abstract}

==> sections/introduction.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%5
%                            INTRODUCTION
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%5

\vspace{3mm}
\section{Introduction}
\label{sec:introduction}

While the vast majority of supervised object detection and segmentation approaches leverage rich datasets with semantically labelled categories, unsupervised methods cannot rely on such a luxury.
Indeed they are expected to infer from the image content itself what is a relevant object and which are its boundaries. This is a daunting task, as relevance is totally domain-specific and also highly subjective, especially when taking in account human judgement, which exploits a lot of out-of-band information that cannot be found in the sheer image data.

As a matter of fact, little effort have been put to investigate unsupervised automatic approaches to detect and segment semantically relevant objects without any additional information than the image or any \textit{a priori} knowledge of the context. This is due to the fact that a unique definition of what is a relevant object (or, how we prefer to call it, a \emph{visual category}) does not actually exist.

This is especially true if we are seeking to set a formal definition that can be adopted across all the domains in a consistent manner with respect to human judgement.  

Within this paper, we try to address this problem by considering a visual category each pattern which appearance is consistent enough across the image. In other words, we consider something to be a relevant object if it appears more than once, exhibiting consistent visual features in different parts of the scene.

\begin{figure}[t]
  \centering
  \includegraphics[width=1\linewidth]{figures/frontpage.jpg}
  \caption{A real world example of unsupervised segmentation of a grocery shelf. Our method can automatically discover both low-level coherent patterns (brands, flavor images and logos) and high-level compound objects (multi-packs and bricks) by controlling the semantical level of the detection and segmentation process.}
  \label{fig:frontpage}
\end{figure}

From a cognitive and perceptual point of view this makes a lot of sense. In fact, it is easy to observe that if a human is presented with images representing several different but recurring objects, even in a cluttered scene, he does not need to know what the objects actually are representing in order to be able to assign semantically-consistent labels to each of them. He would even be able to label each pixel, defining the boundaries of the objects.

As an example, if someone takes a look at a large bin of different (but to some extent repeated) mechanical parts he never saw before, he is still able to tell one part from the other by exploiting their coherent visual and structural appearance.
This ability is also preserved with slight changes in scale, orientation or partial occlusion of the objects.

Since this automatic assignment to a visual category of recurrent object is both well-defined and quite natural in humans, it is a very good candidate as a rule for automatically detecting relevant objects in an unsupervised manner that has good chances of being coherent with human judgement applied to the same image. 

To be fair, we must also underline the fact that, in order to define the boundaries of a visual category and thus obtain a meaningful segmentation, also the level of detail must be taken into account.

As an example, if we present to a human an image of a crowded road captured from a side, and we ask him to segment visual categories according to recurrent patterns, we could get slightly different results from different people depending on their attention to details. Some people will segment cars and trees. Other could consider the car body to be a different object from the wheels ad branches from the tree trunk. The most picky could even separate tires from wheel rims and segment out each single leaf. In practice semantic consistency can happen at different scale when dealing with compound objects presenting themselves internal self repetitions or made up of single parts that are also present in other objects.

To address this aspect we also have to design a proper strategy to perform visual category detection and interpretation at a particular scale, according to the level of detail we want to express during the segmentation process. We define this level of detail as \emph{semantical level}. Semantical levels, of course, do not map directly on specific high level concepts, such as whole objects, large parts or minute components. Rather the semantic level will act as a coarse degree of granularity of the segmentation process that will result in a hierarchical split of segments as it changes.

These two definitions of \emph{visual categories} and \emph{semantical levels}, that will be developed throughout the remainder of the paper, are the two key concepts driving our novel segmentation method.

The ability of our approach to leverage repetitions to capture the internal representation in the real world and then extrapolates visual categories at a specific semantical level is actually achieved through the combination of a couple of standard techniques, slightly modified for the specific task, and of a few key steps specifically crafted to make the process work in a consistent way with respect to the cognitive process adopted by humans. This happens, for instance, by seeking for highly relevant repetitive structural patterns, called \emph{semantical hotspots}, characterized by a novel feature descriptor, called \emph{splash}. We do this through a scale-invariant method and with no continuous geometrical constraints on the visual pattern disposition. 

We also do not constrain ourselves to find only one visual pattern, which is another very common assumption with other approaches in literature. Rather our technique is designed from the start to be able to detect more patterns at once, being able to assign to each of them a different visual category label, corresponding to a different real world object or object part, according to the selected semantical level.

\pagebreak

Overall, with this paper, we are offering to the community the following contributions: 

\begin{itemize}
    \item A new pipeline, including the definition of a specially crafted feature descriptor, to capture semantical categories with the ability to hierarchically span over semantical levels;
    \item A specially crafted conceptual framework to evaluate unsupervised semantic-driven segmentation methods through the introduction of the semantical levels notion along with a new metric;
    \item A new dataset consisting of a few hundredths labelled images that can be used as a benchmark for visual repetition detection in general. 
\end{itemize}

The remainder of the paper is organized as follows. Section \ref{sec:relatedworks} describes the related works with respect to feature extraction and automatic visual patterns detection. Section \ref{sec:methoddescription} introduces our method, giving details on the overall pipeline and on the implementation details. Section \ref{sec:experimental} presents an experimental evaluation and comparison with similar approaches. Finally, the conclusions are found in Section \ref{sec:conclusions}. 

Code, dataset and notebooks used in this paper will be made available for public use.

%In supervised methods, features and mere sintactical properties do not hold any valuable knowledge alone, they acquire significance when hardwired inside the model through the training procedure. 

%What makes our approach particularly appealing is the ability to span over semantical levels, this allows us to get closer on how humans percieve world, in attention-based semantical levls vaben ti ga capio
